Krylov-subspace recycling via the POD-augmented conjugate-gradient method

This work presents a new Krylov-subspace-recycling method for efficiently solving sequences of linear systems of equations characterized by varying right-hand sides and symmetric-positive-definite matrices. As opposed to typical truncation strategies used in recycling such as deflation, we propose a truncation method inspired by goal-oriented proper orthogonal decomposition (POD) from model reduction. This idea is based on the observation that model reduction aims to compute a low-dimensional subspace that contains an accurate solution; as such, we expect the proposed method to generate a low-dimensional subspace that is well suited for computing solutions that can satisfy inexact tolerances. In particular, we propose specific goal-oriented POD `ingredients' that align the optimality properties of POD with the objective of Krylov-subspace recycling. To compute solutions in the resulting `augmented' POD subspace, we propose a hybrid direct/iterative three-stage method that leverages 1) the optimal ordering of POD basis vectors, and 2) well-conditioned reduced matrices. Numerical experiments performed on solid-mechanics problems highlight te benefits of the proposed method over existing approaches for Krylov-subspace recycling.

==> Invariant.tex <==
\begin{theorem}[Distance between goal-oriented POD subspaces]\label{thm:podDistanceGen}
The distance between two goal-oriented POD subspaces
$\podSubspaceIdealShort\defeq\podSubspaceIdeal$ and
$\podSubspacePracticalShort\defeq\podSubspacePractical$---which are characterized by different
metrics 
$\myIdealMetric\in\spsd{\ndof}$ 
and 
$\myPracticalMetric\in\spsd{\ndof}$ 
with $\myIdealMetric
= \myPracticalMetric + \myMetricPerturb$
and different snapshot weights 
$\myIdealEtaMatrix{j}\defeq\diag\totuple{\weightEntryIdeal}{\nsnapshots}$
and
$\myPracticalEtaMatrix{j}\defeq\diag\totuple{\weightEntryPractical}{\nsnapshots}$ 
associated with snapshots
$\myZ{j-1}\in\RR{\ndof\times\nsnapshots}$---can be bounded as
\begin{align} \label{eq:subspaceDistanceBound}
 \distanceMetric{\podSubspaceIdealShort}{\podSubspacePracticalShort}
\le\kappa(\myZ{j-1} \myIdealEtaMatrix{j}) \kappa([\myIdealEtaMatrix{j}]^{-1} \myPracticalEtaMatrix{j}
\myPracticalTruncatedX{j}) \Bigl(&\| 
 \left(\myPracticalEtaMatrix{j} +
\myIdealEtaMatrix{j}\right)\left(\myPracticalEtaMatrix{j} -
\myIdealEtaMatrix{j}\right)[\myIdealEtaMatrix{j}]^{-1} \myZ{j-1}^T
\myPracticalMetric \myZ{j-1} \myIdealEtaMatrix{j} \|_2 \\
& + \| \myMetricPerturb
\|_2 \| \myZ{j-1} \myIdealEtaMatrix{j} \|^2_2\Bigr)/
\text{abssep}(\myPerpIdealTruncatedLambda{j},\myPracticalTruncatedLambda{j})
\end{align}
if the matrix $\myZ{j-1}
\myIdealEtaMatrix{j}$ has full column rank.
Here, $\distanceMetric{\mathcal U}{\mathcal V}\defeq \max_{u\in\mathcal
U, \|u\|=1}{\min_{v\in\mathcal V}}\|u - v\| = \sin(\theta_\text{max})$, where
$\theta_\text{max}$ is the largest principal angle between $\mathcal U$ and $\mathcal
V$, $\kappa(\A)$ denotes the condition number of matrix $\A$, and $
\text{abssep}(\boldsymbol\Lambda_1,\boldsymbol\Lambda_2)\defeq
\min_{\|\boldsymbol Z\|_2 = 1}\|\boldsymbol \Lambda_1 \boldsymbol Z -
\boldsymbol Z\boldsymbol\Lambda_2\|_2
$ denotes the absolute separation between two spectra.
In addition, 
$\myPracticalTruncatedX{j}\in\stiefel{\myTruncDimension}{\mySnapDimension}$
and $\myPracticalTruncatedLambda{j}\in\RR{\myTruncDimension\times\myTruncDimension}$
denote the first $\augSpaceDim$ eigenvectors and (diagonal matrix of) eigenvalues, respectively,
of the matrix
$\myPracticalEtaMatrix{j} \myZ{j-1}^T \myPracticalMetric \myZ{j-1}
\myPracticalEtaMatrix{j}$, assuming eigenvalues are ordered in descending
magnitude.
Similarly, $\myPerpIdealTruncatedLambda{j}$ denotes
the diagonal matrix of eigenvalues associated with 
the orthogonal complement to the
invariant subspace spanned by the first $\augSpaceDim$ eigenvectors of $\myIdealEtaMatrix{j} \myZ{j-1}^T  
\myIdealMetric \myZ{j-1} \myIdealEtaMatrix{j}$.
\end{theorem}

This theorem allows us to bound the distances between the four computable POD
subspaces and their ideal counterparts by substituting the appropriate
quantities into Theorem \ref{thm:podDistanceGen}.
That is, the theorem allows us to bound the following quantities:
\begin{enumerate} 
\item\label{distanceone}
$\distanceMetric{\podSubspace{\augSpaceDim}{\currentDatajm}{\augSpaceWeightsVecPrev}{\Ajm}}{\podSubspace{\augSpaceDim}{\currentDatajm}{\augSpaceWeightsAjVec}{\Aj}}$,
\item\label{distancetwo}
$\distanceMetric{\podSubspace{\augSpaceDim}{\currentDatajm}{\augSpaceWeightsVecRBF(\memory)}{\Ajm}}{\podSubspace{\augSpaceDim}{\currentDatajm}{\augSpaceWeightsAjVec}{\Aj}}$,
\item\label{distancethree}
$\distanceMetric{\podSubspace{\augSpaceDim}{\currentDatajm}{\augSpaceWeightsVecPrev}{\outputMat^T\outputMat}}{\podSubspace{\augSpaceDim}{\currentDatajm}{\augSpaceWeightsAjVec}{\outputMat^T\outputMat}}$,
and
\item\label{distancefour}
$\distanceMetric{\podSubspace{\augSpaceDim}{\currentDatajm}{\augSpaceWeightsVecRBF(\memory)}{\outputMat^T\outputMat}}{\podSubspace{\augSpaceDim}{\currentDatajm}{\augSpaceWeightsAjVec}{\outputMat^T\outputMat}}$.
\end{enumerate}
\begin{remarkk}
\label{rem:subspaceDistance}
The subspace-distance bound \eqref{eq:subspaceDistanceBound}
simplifies under certain conditions. \\
\textit{Fixed snapshot weights.}
First, note that when the snapshot weights are identical but the metric
differes, i.e., 
$\myPracticalEtaMatrix{j} = \myIdealEtaMatrix{j}$, the first term within parentheses vanishes and 
$\kappa([\myIdealEtaMatrix{j}]^{-1} \myPracticalEtaMatrix{j}
\myPracticalTruncatedX{j})=1
$ due to symmetry of $\myGeneralPractical$, which yields
\begin{align} \label{eq:subspaceDistanceBoundMetricOnly}
 \distanceMetric{\podSubspaceIdealShort}{\podSubspacePracticalShort}
\le\kappa(\myZ{j-1} \myIdealEtaMatrix{j}) 
 \| \myMetricPerturb
\|_2 \| \myZ{j-1} \myIdealEtaMatrix{j} \|^2_2/
\text{abssep}(\myPerpIdealTruncatedLambda{j},\myPracticalTruncatedLambda{j}).
\end{align}
Thus, the subspace distance depends linearly on the norm of the metric
perturbation in this case.

\noindent \textit{Fixed metric.} If instead the snapshot weights differ while $\myMetricPerturb = {\bf 0}$, then 
the second term within parentheses vanishes and we have
\begin{align} \label{eq:subspaceDistanceBoundWeightsOnly}
 \distanceMetric{\podSubspaceIdealShort}{\podSubspacePracticalShort}
\le\kappa(\myZ{j-1} \myIdealEtaMatrix{j}) \kappa([\myIdealEtaMatrix{j}]^{-1} \myPracticalEtaMatrix{j}
\myPracticalTruncatedX{j}) &\| 
\left(\myPracticalEtaMatrix{j} +
\myIdealEtaMatrix{j}\right)\left(\myPracticalEtaMatrix{j} -
\myIdealEtaMatrix{j}\right)[\myIdealEtaMatrix{j}]^{-1} \myZ{j-1}^T
\myPracticalMetric \myZ{j-1} \myIdealEtaMatrix{j} \|_2 
/
\text{abssep}(\myPerpIdealTruncatedLambda{j},\myPracticalTruncatedLambda{j})
\end{align}
In practice, this situation corresponds to cases
\ref{distancethree}--\ref{distancefour} above (where 
$\myPracticalMetric =\myIdealMetric= \myCC$) or to cases
\ref{distanceone}--\ref{distancetwo} when 
$\myA{j} = \myA{j-1}$.
Notice that the relative weight perturbation $(\myPracticalEtaMatrix{j} -
\myIdealEtaMatrix{j})[\myIdealEtaMatrix{j}]^{-1}$
appears within the remaining term. When the relative weight perturbation can
be bounded as
$$
\max_k{(\myPracticalEta{j} - \myIdealEta{j})_k / (\myIdealEta{j})_k} \le \myRelativeWeightBound ,
$$
then it can be shown that the bound simplifies to 
\begin{align} \label{eq:subspaceDistanceBoundWeightsOnlyRelFix}
 \distanceMetric{\podSubspaceIdealShort}{\podSubspacePracticalShort}
\le\kappa(\myZ{j-1} \myIdealEtaMatrix{j}) \kappa([\myIdealEtaMatrix{j}]^{-1} \myPracticalEtaMatrix{j}
\myPracticalTruncatedX{j}) &\myRelativeWeightBound (2 +
\myRelativeWeightBound) \| \myIdealEtaMatrix{j} \myZ{j-1}^T \myIdealMetric
\myZ{j-1} \myIdealEtaMatrix{j} \|_2
/
\text{abssep}(\myPerpIdealTruncatedLambda{j},\myPracticalTruncatedLambda{j}).
\end{align}
Further, when 
$\myIdealEtaMatrix{j}$ commutes with $\myZ{j-1}^T \myPracticalMetric \myZ{j-1}$, then the bound simplifies to 
\begin{align} \label{eq:subspaceDistanceBoundWeightsOnlyCommutes}
 \distanceMetric{\podSubspaceIdealShort}{\podSubspacePracticalShort}
\le\kappa(\myZ{j-1} \myIdealEtaMatrix{j}) \kappa([\myIdealEtaMatrix{j}]^{-1} \myPracticalEtaMatrix{j}
\myPracticalTruncatedX{j}) &\| 
\left(\myPracticalEtaMatrix{j} +
\myIdealEtaMatrix{j}\right)\left(\myPracticalEtaMatrix{j} -
\myIdealEtaMatrix{j}\right)  \myZ{j-1}^T
\myPracticalMetric \myZ{j-1}  \|_2 
/
\text{abssep}(\myPerpIdealTruncatedLambda{j},\myPracticalTruncatedLambda{j}),
\end{align}
which now depends on the absolute weight perturbation,
$\myPracticalEtaMatrix{j} - \myIdealEtaMatrix{j}$, rather than
a relative perturbation. This occurs for cases
\ref{distanceone}--\ref{distancetwo} above when $\A_1=\cdots=\Aj=\A$
(i.e., an invariant matrix),
as  $\myZ{j-1}^T \myPracticalMetric \myZ{j-1}$ is diagonal due to enforced $\A$-orthogonality of $\myZ{j-1}$.

\noindent \textit{Strongly separated eigenvalues.} If the eigenvalues associated with 
$\myPracticalTruncatedLambda{j}$ and $\myPerpIdealTruncatedLambda{j}$ in Theorem \ref{thm:podDistanceGen} are strongly separated, i.e., 
$$0<\delta_a\defeq\max\{\min_{\lambda\in\myPracticalTruncatedLambda{j}}|\lambda|-\max_{\hat\lambda\in\myPerpIdealTruncatedLambda{j}}|\hat
\lambda|, \min_{\hat\lambda \in\myPerpIdealTruncatedLambda{j}}|\hat
\lambda| - \max_{\lambda\in\myPracticalTruncatedLambda{j}}|\lambda|\}$$
then the expression for the subspace-distance bound becomes \cite[Theorem 5.3]{ipsen2000absolute}
\begin{align} \label{eq:subspaceDistanceBoundNoAbsSep}
 \distanceMetric{\podSubspaceIdealShort}{\podSubspacePracticalShort}
\le\kappa(\myZ{j-1} \myIdealEtaMatrix{j}) \kappa([\myIdealEtaMatrix{j}]^{-1} \myPracticalEtaMatrix{j}
\myPracticalTruncatedX{j}) \Bigl(&\| 
 \left(\myPracticalEtaMatrix{j} +
\myIdealEtaMatrix{j}\right)\left(\myPracticalEtaMatrix{j} -
\myIdealEtaMatrix{j}\right)[\myIdealEtaMatrix{j}]^{-1} \myZ{j-1}^T
\myPracticalMetric \myZ{j-1} \myIdealEtaMatrix{j} \|_2 \\
& + \| \myMetricPerturb
\|_2 \| \myZ{j-1} \myIdealEtaMatrix{j} \|^2_2\Bigr)/
\delta_a.
\end{align}

Finally, we note that we can apply the results in Eq.~\eqref{eq:weightsDiffAj}
from Theorem \ref{weightsDifference} to those of
Theorem \ref{thm:podDistanceGen} via the triangle inequality to obtain a more
explicit subspace-distance bound for case \ref{distanceone} above, where 
$\myIdealEtaMatrix{j} = \diag\totuple{[\augSpaceWeightsAjVec]}{\nsnapshots}$
and $\myPracticalEtaMatrix{j} = 
\diag\totuple{\augSpaceWeightsEntryPrev}{\nsnapshots}$.
\end{remarkk}


==> abstract.tex <==
This work presents a new Krylov-subspace-recycling method for efficiently solving sequences of linear systems of equations characterized by varying right-hand sides and symmetric-positive-definite matrices. As opposed to typical truncation strategies used in recycling such as deflation, we propose a truncation method inspired by goal-oriented proper orthogonal decomposition (POD) from model reduction.  This idea is based on the observation that model reduction aims to compute a low-dimensional subspace that contains an \textit{accurate} solution; as such, we expect the proposed method to generate a low-dimensional subspace that is well suited for computing solutions that can satisfy \textit{inexact} tolerances. In particular, we propose specific goal-oriented POD `ingredients' that align the optimality properties of POD with the objective of Krylov-subspace recycling.  To compute solutions in the resulting `augmented' POD subspace, we propose a hybrid direct/iterative three-stage method that leverages 1) the optimal ordering of POD basis vectors, and 2) well-conditioned reduced matrices. Numerical experiments performed on solid-mechanics problems highlight the benefits of the proposed method over existing approaches for Krylov-subspace recycling.


==> aug_kry_algorithm_general2.tex <==
\begin{algorithm}[htbp]
\caption{ \stagetwoalgorithmname }
\begin{algorithmic}[1]\label{alg:augmentedCGgen}
\small
\REQUIRE $\A$, $\b$, $\xArgHat{0}$, $\augSpaceBasis$, $\prec$, 
 $\tol$
\ENSURE $\kitNo$, $\alphaVec$, $\kryVec$, $\vecLengthAll$  %$\redstate^{\timestepit}$
%\STATE\label{step:solveRom} Compute ROM solution $\redstate^{\timestepit}$
%satisfying
\STATE $\xArg{0} = \augSpaceBasis\xArgHat{0}$
\STATE $\rArg{0} = \b - \A\xArg{0}$
\STATE $\zArg{0} = \precInv \rArg{0}$
\STATE \label{step:aug2}Solve $\augSpaceBasis^T \A   \augSpaceBasis\augComponentArg{0} =
\augSpaceBasis^T \A  \zArg{0}$. 
\STATE\label{step:aug2part2} $\pArg{0} = \zArg{0} - \augSpaceBasis\augComponentArg{0} $
\FOR{$k = 0, 1, \ldots$}
\STATE $\vecLengthArg{k} = (\A\pArg{k},\pArg{k})$
\STATE  $\alphaArg{k} = (\rArg{k},\zArg{k})/\vecLengthArg{k}$
\STATE  $\xArg{k+1} = \xArg{k} + \alphaArg{k} \pArg{k} $
\STATE\label{step:res}  $\rArg{k+1} = \rArg{k} - \alphaArg{k} \A  \pArg{k}$
\STATE  $\zArg{k+1} = \precInv\rArg{k+1}$
\STATE  $\beta^{(k+1)} = \frac{(\rArg{k+1},\zArg{k+1})}{(\rArg{k},\zArg{k})}$
\STATE  \label{step:aug3}Solve $\augSpaceBasis^T \A  \augSpaceBasis
\augComponentArg{k+1} =
\augSpaceBasis^T \A  \zArg{k+1} $.
\STATE\label{step:aug3part2}  $ \pArg{k+1} = \zArg{k+1} + \beta^{(k+1)} \pArg{k} -
\augSpaceBasis\augComponentArg{k+1}$
\IF{$\|\rArg{k+1}\|\leq \tol$  } 
\STATE Exit.
\ENDIF
 \ENDFOR
 \STATE $\kitNo = k+1$, $\alphaVec =
 \left[\alphaArg{0}\ \cdots\ \alphaArg{k-1}\right]^T$, $\kryVec =
  \left[\pArg{0}\ \cdots\
 \pArg{k-1}\right]$, $\vecLengthAll =
 \diag{(\vecLengthArg{0},\ldots,\vecLengthArg{k-1})}$ 
\end{algorithmic}
\end{algorithm}



==> overall_algorithm.tex <==
\begin{algorithm}[htbp]
\caption{\overallalgorithmname}
\begin{algorithmic}[1]\label{alg:overall}
\small
\REQUIRE $\{\Aj\}_{j=1}^{\nlhs}$,
$\{\bj\}_{j=1}^{\nlhs}$,
$\{\xGuessj\}_{j=1}^{\nlhs}$,
forcing sequence $\{\tolj\}_{j=1}^{\nlhs}$, storage threshold
$\augSpaceThreshold$,
stage-1 option $\newvectorsdirect$, stage-3 option $\stagethreeoptionone$
\ENSURE 
\STATE $\stageonebasisArg{1} \leftarrow \emptyset$,
$\stagetwobasisArg{1}\leftarrow \emptyset$, $\jcompress
\leftarrow 0$
\FOR{$j = 1, \ldots, \nlhs$}
\IF{$\stageonebasisj\neq\emptyset$}
\STATE \textit{Stage 1}: ($\stageonesolredj$, $\cholRedj$) =
\stageonealgorithmname($\Aj$, $\bj - \Aj\xGuessj$,
$\stageonebasisj$)
\ENDIF
\IF{$\stagetwobasisj\neq\emptyset$}
\STATE \textit{Stage 2}: ($\stagetwoitj$, $\stagetwosolredj$,
$\stagetwoaugj$, $\redTj$) = \stagetwoalgorithmname($
\augSpaceBasisj^T\Aj\augSpaceBasisj$, $
\augSpaceBasisj^T(\bj - \Aj\xGuessj)$, 
$\stageonesolredj$,
$\stageoneaugj$, $\I$,  $\tolstagetwoj$).\\
Note optimizations discussed in Section
\ref{sec:stage2}
\ENDIF
\IF[orthogonalize against entire $\augSpaceBasisj$]{$\stagethreeoptionone=$\true}
\STATE \textit{Stage 3}: 
($\kit{j}$, $\redKryj$, $\kryVecj$,
$\Tj$) = \stagetwoalgorithmname(
$\Aj$, $ \bj - \Aj\xGuessj$,
$\stageoneaugj\stageonesolredj+\stagetwoaugj\stagetwosolredj$,
$\augSpaceBasisj$, $\precj$, and $\tolj$).\\ Note optimizations discussed in Section \ref{sec:stage3special}
\ELSE
\STATE \textit{Stage 3}: 
($\kit{j}$,
$\redKryj$, $\kryVecj$,
$\Tj$) = \stagetwoalgorithmname(
$ \Aj$, $ \bj - \Aj\xGuessj$,
$\left[\stageonesolredj^T\ \stagetwosolredj^T\right]^T$,
$[\stageonebasisj\ \stagetwobasisj]$, $
\precj$, $ \tolj$).\\ Note optimizations discussed in Section \ref{sec:stage3}
\ENDIF
\STATE$\stageonebasisArg{j+1} \leftarrow\stageonebasisArg{j}$
\STATE $\stageonesetj \leftarrow \{i\ |\
[\Tj]_{ii}/\sum_{k=1}^{\kit{j}}[\Tj]_{kk} >
\newvectorsdirect \}$
\FOR{$k\in\stageonesetj$}
\STATE $\stageonebasisArg{j+1} \leftarrow[\stageonebasisArg{j+1},\
[\kryVecj]_k\sqrt{[\Tj]_{kk}}]$
\ENDFOR
\IF[include new vectors in stage-1 basis]{$\newvectorsdirect=$\true}
\STATE $\stageonebasisArg{j+1} \leftarrow[\stageonebasisArg{j},\ \kryVecj\sqrt{\Tj}]$
\ELSE
\STATE$\stageonebasisArg{j+1} \leftarrow\stageonebasisArg{j}$
\ENDIF
\IF[truncate]{$\augSpaceDimjp > \augSpaceThreshold$}
\STATE\label{step:compress1} $\augSpaceBasisjp =
\compressionalgorithmname([\augSpaceBasisj,\kryVecj])$ (note that $\currentDataj =[\augSpaceBasisj,\kryVecj]$)
\STATE\label{step:enforceOrthog} Enforce $\Aj$-orthogonality:
$\augSpaceBasisjp^T\Aj\augSpaceBasisjp = \cholEnforcejT\cholEnforcej$
(Cholesky factorization),
$\augSpaceBasisjp\leftarrow \augSpaceBasisjp\cholEnforcejinv$
\STATE\label{step:compresslast} Determine $\stageonebasisArg{j+1}$ with
$\range{\stageonebasisArg{j+1}}\subseteq \range{\augSpaceBasisArg{j+1}}$
\STATE Update lastest-truncation index $\jcompress \leftarrow j$
\ELSE
\STATE $\augSpaceBasisjp \leftarrow \left[\augSpaceBasisj,\ \kryVecj\sqrt{\Tj}\right]$
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}



==> pod_cg_journal_title_siam.tex <==
\title{Krylov-subspace recycling via\\ the POD-augmented conjugate-gradient method}
\author{Kevin Carlberg\thanks{Sandia National Laboratories
(\href{mailto:ktcarlb@sandia.gov}{ktcarlb@sandia.gov},
\href{mailto:rstumin@sandia.gov}{rstumin@sandia.gov}).}
\and Virginia Forstall\thanks{University of Maryland (\href{mailto:vhfors@gmail.com}{vhfors@gmail.com}).}
\and Ray Tuminaro\footnotemark[1]
}%
%{\normalsize\itshape
%Sandia National Laboratories, Livermore, CA 94551, USA\thanks{Sandia National
%Laboratories, P.O. Box 969, MS 9159, Livermore, CA
%94551, USA. Sandia is a multiprogram laboratory operated by Sandia
%Corporation, a Lockheed Martin Company, for the United States Department of
%Energy under contract DE-AC04-94-AL85000.}

